Classifying grounded intersection graphs via ordered forbidden patterns

It was noted already in the 90s that many classic graph classes, such as interval, chordal, and bipartite graphs, can be characterized by the existence of an ordering of the vertices avoiding some ordered subgraphs, called patterns. Very recently, all the classes corresponding to patterns on three vertices (including the ones mentioned above) have been listed, and proved to be efficiently recognizable. In contrast, very little is known about patterns on four vertices. One of the few graph classes characterized by a pattern on four vertices is the class of intersection graphs of rectangles that are said to be grounded on a line. This class appears naturally in the study of intersection graphs, and similar grounded classes have recently attracted a lot of attention. This paper contains three parts. First, we make a survey of grounded intersection graph classes, summarizing all the known inclusions between these various classes. Second, we show that the correspondence between a pattern on four vertices and grounded rectangle graphs is not an isolated phenomenon. We establish several other pattern characterizations for geometric classes, and show that the hierarchy of grounded intersection graph classes is tightly interleaved with the classes defined patterns on four vertices. We claim that forbidden patterns are a useful tool to classify grounded intersection graphs. Finally, we give an overview of the complexity of the recognition of classes defined by forbidden patterns on four vertices and list several interesting open problems.

==> LM.tex <==
\begin{tikzpicture}   
[scale=1.0,auto=left,every node/.style={circle,draw,fill=black!5}]   
\node (n1) at (0,0) {1};   
\node (n2) at (1,0) {2};   
\node (n3) at (2,0)  {3};   
\node (n4) at (3,0)  {4};   
    

\draw (n1) to[bend left=50] (n3); 
\draw (n2) to[bend left=50] (n4); 
\draw[dashed] (n1) to (n2);
\draw[dashed] (n2) to (n3);
\end{tikzpicture}

==> LMR.tex <==
\begin{tikzpicture}   
[scale=1.0,auto=left,every node/.style={circle,draw,fill=black!5}]   
\node (n1) at (0,0) {1};   
\node (n2) at (1,0) {2};   
\node (n3) at (2,0)  {3};   
\node (n4) at (3,0)  {4};   
    

\draw (n1) to[bend left=50] (n3); 
\draw (n2) to[bend left=50] (n4); 
\draw[dashed] (n1) to (n2);
\draw[dashed] (n2) to (n3);
\draw[dashed] (n3) to (n4);
\end{tikzpicture}

==> P0.tex <==
\begin{tikzpicture}   
[scale=0.8,auto=left,every node/.style={circle,draw,fill=black!5}]   
\node (n1) at (0,0) {};   
\node (n2) at (1,0) {};   
\node (n3) at (2,0)  {};   
\node (n4) at (3,0)  {};   
    

\draw (n1) to[bend left=50] (n3); 
\draw (n2) to[bend left=50] (n4);
 
\end{tikzpicture}

==> Pa.tex <==
\begin{tikzpicture}
	[scale=0.8, 
	auto=left,every node/.style
	={circle,draw,fill=black!5}]
	\node (1) at (0,0) {};
	\node (2) at (1,0) {};
	\node (3) at (2,0) {};
	\node (4) at (3,0) {};
	
	\draw[dashed] (1) to node[draw=none, fill=none] {} (2);
	\draw[bend left=50] (1) to (3);
	\draw[bend left=50] (2) to (4) ;
\end{tikzpicture}

==> Pab.tex <==
\begin{tikzpicture}
	[scale=0.8, 
	auto=left,every node/.style
	={circle,draw,fill=black!5}]
	\node (1) at (0,0) {};
	\node (2) at (1,0) {};
	\node (3) at (2,0) {};
	\node (4) at (3,0) {};
	
	\draw[dashed] (1) to node[draw=none, fill=none] {} (2);
	\draw[bend left=50] (1) to (3);
	\draw[dashed] (2) to node[draw=none, fill=none] {} (3) ;
	\draw[bend left=50] (2) to (4) ;
\end{tikzpicture}

==> Pb.tex <==
\begin{tikzpicture}
	[scale=0.8, 
	auto=left,every node/.style
	={circle,draw,fill=black!5}]
	\node (1) at (0,0) {};
	\node (2) at (1,0) {};
	\node (3) at (2,0) {};
	\node (4) at (3,0) {};
	
	\draw[bend left=50] (1) to (3);
	\draw[dashed] (2) to node[draw=none, fill=none] {} (3) ;
	\draw[bend left=50] (2) to (4) ;
\end{tikzpicture}

==> bipartite.tex <==
\begin{tikzpicture}
	[scale=0.7,auto=left,every node/.style=		
	{circle,draw,fill=black!5}]
	\node (a) at (0,0) {};
	\node (b) at (1,0) {};
	\node (c) at (2,0) {};
	\draw (a) to (b);
	\draw (b) to (c);
\end{tikzpicture}

==> chordal.tex <==
\begin{tikzpicture}
	[scale=0.7,auto=left,every node/.style=		
	{circle,draw,fill=black!5}]
	\node (a) at (0,0) {};
	\node (b) at (1,0) {};
	\node (c) at (2,0) {};
	\draw (a) to[bend left=50] (c);
	\draw[dashed] (a) to (b);
	\draw (b) to (c);
\end{tikzpicture}

==> cochordal.tex <==
\begin{tikzpicture}
			[scale=0.7,auto=left,every node/.style=		
			{circle,draw,fill=black!5}]
			\node (a) at (0,0) {};
			\node (b) at (1,0) {};
			\node (c) at (2,0) {};
			\draw[dashed] (a) to[bend left=50] (c);
			\draw (a) to (b);
			\draw[dashed] (b) to (c);
		\end{tikzpicture}

==> cocomparability-2.tex <==
\begin{tikzpicture}
			[scale=1.0,auto=left,every node/.style=		
			{circle,draw,fill=black!5}]
			\node (a) at (0,0) {};
			\node (b) at (1,0) {};
			\node (c) at (2,0) {};
			\draw (a) to[bend left=50] (c);
			\draw[dashed] (a) to (b);
			\draw[dashed] (b) to (c);
		\end{tikzpicture}

==> cointerval.tex <==
\begin{tikzpicture}
			[scale=0.7,auto=left,every node/.style=		
			{circle,draw,fill=black!5}]
			\node (a) at (0,0) {};
			\node (b) at (1,0) {};
			\node (c) at (2,0) {};
			\draw[dashed] (a) to[bend left=50] (c);
			\draw (a) to (b);
		\end{tikzpicture}

==> cross_and_left_missing.tex <==
\begin{tikzpicture}   
[scale=1.0,auto=left,every node/.style={circle,draw,fill=black!5}]   
\node (n1) at (0,0) {1};   
\node (n2) at (1,0) {2};   
\node (n3) at (2,0)  {3};   
\node (n4) at (3,0)  {4};   
    

\draw (n1) to[bend left=50] (n3); 
\draw (n2) to[bend left=50] (n4); 
\draw[dashed] (n1) to (n2);
\end{tikzpicture}

==> diagonal_rectangle.tex <==
\begin{tikzpicture}   
[scale=1.0,auto=left,every node/.style={circle,draw,fill=black!5}]   
\node (n1) at (0,0) {1};   
\node (n2) at (1,0) {2};   
\node (n3) at (2,0)  {3};   
\node (n4) at (3,0)  {4};   
    

\draw (n1) to[bend left=50] (n3); 
\draw (n2) to[bend left=50] (n4);
\draw[dashed] (n2) to (n3);
 
\end{tikzpicture}

==> fig-interval-representations.tex <==
\begin{figure}[!h]
	\begin{center}
			\begin{subfigure}{0.3 \textwidth}
			\centering
			
				\includegraphics[scale=0.3]%
				{ps_pictures/intervalles.eps}
			
			\vspace{0.2cm}
			\caption{\label{fig:interval_inter}Classic intervals graph (shifted for better readability).}
		\end{subfigure}
	%
		\begin{subfigure}{0.3 \textwidth}
			\centering
			
				\scalebox{0.3}{
				\includegraphics[scale=1]{ps_pictures/%
				infinite_rectangles.eps}
				
			}{}
			\caption{\label{fig:infinite_interval}
			Infinite rectangles.}
		\end{subfigure}
	%	
		\begin{subfigure}{0.3 \textwidth}
			\centering
			
				\scalebox{0.3}{
				\includegraphics[scale=1]{ps_pictures/%
				interval_as_planted_on_two_lines.eps}
				
			}{}	
			\caption{\label{fig:interval_as_planted_on_two_lines}
			Intervals as doubly-planted filaments.}
		\end{subfigure}
	
	\caption{\label{fig:intersection_interval} Different intersection representations of interval graphs. First the classic intervals (slightly shifted for readability). Second the grounded representation. Third the two-lines representation. } 
		\end{center}

	\end{figure}

==> fig-perm-cocomp.tex <==
\begin{figure}[!h]	
	%
		\begin{subfigure}{0.5 \textwidth}
			\centering
			
				\includegraphics[scale=1.2]%
				{ps_pictures/permutation.eps}
			{}	
			\vspace{0.2cm}
			\caption{\label{fig:permutation_inter}
			Permutation graph.}
		\end{subfigure}
	%
		\begin{subfigure}{0.5 \textwidth}
			\centering
			
				\includegraphics[scale=0.8]%
				{ps_pictures/cocomp.eps}
			{}
			\vspace{0.2cm}
			\caption{\label{fig:cocomp_inter} 
			Co-comparability graph.}
		\end{subfigure}
	%
	\caption{\label{fig:inter}
	The graph that illustrates the cocomparability graphs is ($\bar{X_{31}}$) that is
	not be comparability graph, thus not a permutation graph. 
	The permutatation one is a 4-cycle, that not an interval graph.} 
	\end{figure}

==> fig-rectangles-and-L.tex <==
\begin{figure}[h!]
	\begin{subfigure}{0.5 \textwidth}
			\centering
				\includegraphics[scale=1]%
				{ps_pictures/rectangles.eps}
			\vspace{0.2cm}
			\caption{\label{fig:rectangles}
			Grounded rectangles.}
		\end{subfigure}
	%
	\begin{subfigure}{0.5 \textwidth}
			\centering
				\includegraphics[scale=0.9]%
				{ps_pictures/L-shape.eps}
			\vspace{0.2cm}
			\caption{\label{fig:L-shape}
			L-shape.}
		\end{subfigure}
	\caption{\label{fig:rectangles-and-L}
	Intersection representations for classes with patterns on four nodes.}
\end{figure}

==> interval.tex <==
\begin{tikzpicture}
			[scale=0.7,auto=left,every node/.style=		
			{circle,draw,fill=black!5}]
			\node (a) at (0,0) {};
			\node (b) at (1,0) {};
			\node (c) at (2,0) {};
			\draw (a) to[bend left=50] (c);
			\draw[dashed] (a) to (b);
		\end{tikzpicture}

==> outerplanar.tex <==
\begin{tikzpicture}   
[scale=1.5,auto=left,every node/.style={circle,draw,fill=black!5}]   
\node (n1) at (0,0) {1};   
\node (n2) at (1,0) {2};   
\node (n3) at (2,0)  {3};   
\node (n4) at (3,0)  {4};   
    

\draw (n1) to[bend left=50] (n3); 
\draw (n2) to[bend left=50] (n4);
 
\end{tikzpicture}

==> reverse_chordal.tex <==
\begin{tikzpicture}
	[scale=0.7,auto=left,every node/.style=		
	{circle,draw,fill=black!5}]
	\node (a) at (0,0) {};
	\node (b) at (1,0) {};
	\node (c) at (2,0) {};
	\draw (a) to[bend left=50] (c);
	\draw (a) to (b);
	\draw[dashed] (b) to (c);
\end{tikzpicture}

==> reverse_interval.tex <==
\begin{tikzpicture}
	[scale=0.7,auto=left,every node/.style=		
	{circle,draw,fill=black!5}]
	\node (a) at (0,0) {};
	\node (b) at (1,0) {};
	\node (c) at (2,0) {};
	\draw (a) to[bend left=50] (c);
	\draw[dashed] (b) to (c);
\end{tikzpicture}

==> rounding-rectangle-trick.tex <==
\makeatletter

\pgfkeys{/pgf/.cd,
 rectangle corner radius/.initial=3pt
}
\newif\ifpgf@rectanglewrc@donecorner@
\def\pgf@rectanglewithroundedcorners@docorner#1#2#3#4{%
  \edef\pgf@marshal{%
    \noexpand\pgfintersectionofpaths
      {%
        \noexpand\pgfpathmoveto{\noexpand\pgfpoint{\the\pgf@xa}{\the\pgf@ya}}%
        \noexpand\pgfpathlineto{\noexpand\pgfpoint{\the\pgf@x}{\the\pgf@y}}%
      }%
      {%
        \noexpand\pgfpathmoveto{\noexpand\pgfpointadd
          {\noexpand\pgfpoint{\the\pgf@xc}{\the\pgf@yc}}%
          {\noexpand\pgfpoint{#1}{#2}}}%
        \noexpand\pgfpatharc{#3}{#4}{\cornerradius}%
      }%
    }%
  \pgf@process{\pgf@marshal\pgfpointintersectionsolution{1}}%
  \pgf@process{\pgftransforminvert\pgfpointtransformed{}}%
  \pgf@rectanglewrc@donecorner@true
}
\pgfdeclareshape{rectangle with rounded corners}
{
  \inheritsavedanchors[from=rectangle] % this is nearly a rectangle
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{mid east}
  \inheritanchor[from=rectangle]{base}
  \inheritanchor[from=rectangle]{base west}
  \inheritanchor[from=rectangle]{base east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}

  \savedmacro\cornerradius{%
    \edef\cornerradius{\pgfkeysvalueof{/pgf/rectangle corner radius}}%
  }

  \backgroundpath{%
    \northeast\advance\pgf@y-\cornerradius\relax
    \pgfpathmoveto{}%
    \pgfpatharc{0}{90}{\cornerradius}%
    \northeast\pgf@ya=\pgf@y\southwest\advance\pgf@x\cornerradius\relax\pgf@y=\pgf@ya
    \pgfpathlineto{}%
    \pgfpatharc{90}{180}{\cornerradius}%
    \southwest\advance\pgf@y\cornerradius\relax
    \pgfpathlineto{}%
    \pgfpatharc{180}{270}{\cornerradius}%
    \northeast\pgf@xa=\pgf@x\advance\pgf@xa-\cornerradius\southwest\pgf@x=\pgf@xa
    \pgfpathlineto{}%
    \pgfpatharc{270}{360}{\cornerradius}%
    \northeast\advance\pgf@y-\cornerradius\relax
    \pgfpathlineto{}%
  }

  \anchor{before north east}{\northeast\advance\pgf@y-\cornerradius}
  \anchor{after north east}{\northeast\advance\pgf@x-\cornerradius}
  \anchor{before north west}{\southwest\pgf@xa=\pgf@x\advance\pgf@xa\cornerradius
    \northeast\pgf@x=\pgf@xa}
  \anchor{after north west}{\northeast\pgf@ya=\pgf@y\advance\pgf@ya-\cornerradius
    \southwest\pgf@y=\pgf@ya}
  \anchor{before south west}{\southwest\advance\pgf@y\cornerradius}
  \anchor{after south west}{\southwest\advance\pgf@x\cornerradius}
  \anchor{before south east}{\northeast\pgf@xa=\pgf@x\advance\pgf@xa-\cornerradius
    \southwest\pgf@x=\pgf@xa}
  \anchor{after south east}{\southwest\pgf@ya=\pgf@y\advance\pgf@ya\cornerradius
    \northeast\pgf@y=\pgf@ya}

  \anchorborder{%
    \pgf@xb=\pgf@x% xb/yb is target
    \pgf@yb=\pgf@y%
    \southwest%
    \pgf@xa=\pgf@x% xa/ya is se
    \pgf@ya=\pgf@y%
    \northeast%
    \advance\pgf@x by-\pgf@xa%
    \advance\pgf@y by-\pgf@ya%
    \pgf@xc=.5\pgf@x% x/y is half width/height
    \pgf@yc=.5\pgf@y%
    \advance\pgf@xa by\pgf@xc% xa/ya becomes center
    \advance\pgf@ya by\pgf@yc%
    \edef\pgf@marshal{%
      \noexpand\pgfpointborderrectangle
      {\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}
      {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
    }%
    \pgf@process{\pgf@marshal}%
    \advance\pgf@x by\pgf@xa% 
    \advance\pgf@y by\pgf@ya%
    \pgfextract@process\borderpoint{}%
    %
    \pgf@rectanglewrc@donecorner@false
    %
    % do southwest corner
    \southwest\pgf@xc=\pgf@x\pgf@yc=\pgf@y
    \advance\pgf@xc\cornerradius\relax\advance\pgf@yc\cornerradius\relax 
    \borderpoint
    \ifdim\pgf@x<\pgf@xc\relax\ifdim\pgf@y<\pgf@yc\relax
      \pgf@rectanglewithroundedcorners@docorner{-\cornerradius}{0pt}{180}{270}%
    \fi\fi
    %
    % do southeast corner
    \ifpgf@rectanglewrc@donecorner@\else
      \southwest\pgf@yc=\pgf@y\relax\northeast\pgf@xc=\pgf@x\relax
      \advance\pgf@xc-\cornerradius\relax\advance\pgf@yc\cornerradius\relax
      \borderpoint
      \ifdim\pgf@x>\pgf@xc\relax\ifdim\pgf@y<\pgf@yc\relax
       \pgf@rectanglewithroundedcorners@docorner{0pt}{-\cornerradius}{270}{360}%
      \fi\fi
    \fi
    %
    % do northeast corner
    \ifpgf@rectanglewrc@donecorner@\else
      \northeast\pgf@xc=\pgf@x\relax\pgf@yc=\pgf@y\relax
      \advance\pgf@xc-\cornerradius\relax\advance\pgf@yc-\cornerradius\relax
      \borderpoint
      \ifdim\pgf@x>\pgf@xc\relax\ifdim\pgf@y>\pgf@yc\relax
       \pgf@rectanglewithroundedcorners@docorner{\cornerradius}{0pt}{0}{90}%
      \fi\fi
    \fi
    %
    % do northwest corner
    \ifpgf@rectanglewrc@donecorner@\else
      \northeast\pgf@yc=\pgf@y\relax\southwest\pgf@xc=\pgf@x\relax
      \advance\pgf@xc\cornerradius\relax\advance\pgf@yc-\cornerradius\relax
      \borderpoint
      \ifdim\pgf@x<\pgf@xc\relax\ifdim\pgf@y>\pgf@yc\relax
       \pgf@rectanglewithroundedcorners@docorner{0pt}{\cornerradius}{90}{180}%
      \fi\fi
    \fi
  }
}

\makeatother

%\begin{tikzpicture}
%  \draw node(rc)[
%    rectangle with rounded corners,draw,rectangle corner radius=10pt,align=center]
%    {\large rectangle with rounded corners\\\large rectangle with rounded corners\\\large rectangle with rounded corners};
%  \fill[red,every node/.style={font=\tiny}]
%        \foreach \d/\p in {before north east/right,after north east/above,
%                           before north west/above,after north west/left,
%                           before south west/left,after south west/below,
%                           before south east/right,after south east/right}
%                       { (rc.\d) circle(1pt) node[\p]{\d} };
%  \draw[blue,draw opacity=0.3]\foreach\a in {0,...,360} {(rc)--+(\a:5cm)};
%\end{tikzpicture}
%
%\end{document}

==> split-3.tex <==
\begin{tikzpicture}[scale=0.7, auto=left, every node/.style=	{circle,draw,fill=black!5}]
	\node (a) at (0,0) {};
	\node (b) at (1,0) {};
	\node (c) at (2,0) {};
	\draw (a) to (b);
	\draw[dashed] (b) to (c);
\end{tikzpicture}

==> star.tex <==
\begin{tikzpicture}[scale=0.7,auto=left,every node/.style=	 {circle, draw, fill=black!5}]
	\node (a) at (0,0) {};
	\node (b) at (1,0) {};
	\node (c) at (2,0) {};
	\draw (a) to (b);

\end{tikzpicture}

==> three-colorable.tex <==
\begin{tikzpicture}
	[scale=0.7,auto=left,every node/.style=		
	{circle,draw,fill=black!5}]
	%\filldraw[fill=g6, rounded corners=8pt] (-1,-0.8) rectangle (4,0.8);
	\node (a) at (0,0) {};
	\node (b) at (1,0) {};
	\node (c) at (2,0) {};
	\node (d) at (3,0) {};
	\draw[line width=0.04cm] (a) to (b);
	\draw[line width=0.04cm] (b) to (c);
	\draw[line width=0.04cm] (c) to (d);
\end{tikzpicture}

==> tree.tex <==
\begin{tikzpicture}
			[scale=0.7,auto=left,every node/.style=		
			{circle,draw,fill=black!5}]
			\node (a) at (0,0) {};
			\node (b) at (1,0) {};
			\node (c) at (2,0) {};
			\draw (a) to[bend left=50] (c);
			\draw (b) to (c);
		\end{tikzpicture}

==> trianglefree.tex <==
\begin{tikzpicture}
			[scale=0.7,auto=left,every node/.style=		
			{circle,draw,fill=black!5}]
			\node (a) at (0,0) {};
			\node (b) at (1,0) {};
			\node (c) at (2,0) {};
			\draw (a) to[bend left=50] (c);
			\draw (a) to (b);
			\draw (b) to (c);
		\end{tikzpicture}
